Feature Incay for Representation Regularization

Softmax loss is widely used in deep neural networks for multi-class classification, where each class is represented by a weight vector, a sample is represented as a feature vector, and the feature vector has the largest projection on the weight vector of the correct category when the model correctly classifies a sample. To ensure generalization, weight decay that shrinks the weight norm is often used as regularizer. Different from traditional learning algorithms where features are fixed and only weights are tunable, features are also tunable as representation learning in deep learning. Thus, we propose feature incay to also regularize representation learning, which favors feature vectors with large norm when the samples can be correctly classified. With the feature incay, feature vectors are further pushed away from the origin along the direction of their corresponding weight vectors, which achieves better inter-class separability. In addition, the proposed feature incay encourages intra-class compactness along the directions of weight vectors by increasing the small feature norm faster than the large ones. Empirical results on MNIST, CIFAR10 and CIFAR100 demonstrate feature incay can improve the generalization ability.

==> Makefile <==
# Copyright (c) 2008-2009 solvethis
# Copyright (c) 2010-2012 Casper Ti. Vector
# Public domain.

# 被编译的主文件的文件名，不包括扩展名。
JOBNAME = nips_2017
# 这个变量的值可以为 latex、pdflatex 或 xelatex。
LATEX = pdflatex
# BIBTEX = biber -l zh__pinyin
DVIPDF = dvipdfmx

# 如果用 LaTeX 编译，则使用 dvipdfmx 将 dvi 转成 pdf。
ifeq ($(LATEX), latex)
	DODVIPDF = $(DVIPDF) $(JOBNAME)
endif

# 区分是 Windows 环境还是类 UNIX 环境。
# 如果是后者，则 GNU make 将可以检测到已经定义 PATH 环境变量。
ifdef PATH
	MAKE = make
	RM = rm -f
else
	MAKE = mingw32-make
	RM = del
endif

doc:
	$(LATEX) $(JOBNAME)
	$(BIBTEX) $(JOBNAME)
	# $(LATEX) $(JOBNAME)
	# $(LATEX) $(JOBNAME)
	# $(BIBTEX) $(JOBNAME)
	# $(DODVIPDF)

clean:
	$(RM) $(JOBNAME).{aux,bbl,bcf,blg,dvi,lof,log,lot,run.xml,toc,out{,.bak}} \
		{missfont,texput}.log 

distclean: clean
	$(RM) $(JOBNAME).pdf

# vim:ts=4:sw=4


==> chap/old_our_work.tex <==
\section{Our work}
\subsection{Large $\emph{L}_{2}$-norm Softmax Loss}
We propose the novel Large $\emph{L}_{2}$-norm Softmax Loss mainly based on the following property, which is similar to the proposition 1 in~\cite{wang2017normface}.\\

\textbf{Proposition 3.1} \emph{Fixing the $\emph{L}_{2}$-norm of weight vectors constant and ignoring the bias vectors, the Softmax loss is a monotonically decreasing function with the decreasing of the angles between the features $f_i$  and its corresponding weight vectors $w_{y_i}$ if the $x_{i}$ has been correctly classified.}
y constraining the $\| w_{k} \| \equiv 1$ and $b_{k} \equiv 0$ for all $k=1 \cdots K$in equation\eqref{softmax_loss_cos}, we get .
\begin{footnotesize}
\begin{align}
\mathcal{L}_{Softmax}(k, f_k)&=-log\bigg( \frac {exp(\| w_{y_k} \| \| f_{k} \| cos({\theta}_{w_{y_k}, f_{k}}) + b_{y_k})} {\sum_{j=1}^{K}exp(\| w_{j} \| \| f_{k} \| cos({\theta}_{w_{j}, f_{k}}) + b_k)} \bigg)  \notag \\
&= -log\bigg( \frac {1} {\sum_{j=1}^{K}exp(\| f_{k} \| (\| w_{j} \| cos({\theta}_{w_{j}, f_{k}}) + b_k - \| w_{y_k} \| cos({\theta}_{w_{y_k}, f_{k}}) - b_{y_k}))} \bigg)
\end{align}
\end{footnotesize}

Recall that the $x_{k}$ is correctly classfied, so we have $w_{y_k}f_{k}+b_{y_k} > w_{j}f_{k}+b_{j}$ for any $j \neq y_{k}$. Then $\| f_{k} \| (\| w_{j} \| cos({\theta}_{w_{j}, f_{k}}) + b_k - \| w_{y_k} \| cos({\theta}_{w_{y_k}, f_{k}}) - b_{y_k}) < 0$ always holds. So we have for any $t > 0$,  

% \textbf{Property} \emph{For the softmax loss with no-bias inner-product similarity as its metric, let $P_{i}(f) = \frac{e^{w_{i}^{T}f}}{\sum_{j=1}^{K}e^{w_{j}^{T}f}})$ denote the probability of \textbf{f} being classified as class i. For a given scale s > 1, if $i = argmax_{j}(w_{j}^{T}f)$, then $P_{i}(sf) \ge P_{i}(f)$ always holds.}




\begin{align}
\mathcal{L}_{Softmax}(k, (1 + t)f_k) < \mathcal{L}_{Softmax}(k, f_k)
\end{align}
if we keep the $\| w_{j} \|$ and $cos({\theta}_{w_{j}, f_{k}})$ fixed. By considering all the $x_{i}$, we have ($t_k > 0$ for $k = 1 \cdots N$)
\begin{align}
\sum_{k=1}^{N} \mathcal{L}_{Softmax}(k, (1 + t_k)f_k) < \sum_{k=1}^{N} \mathcal{L}_{Softmax}(k, f_k)
\end{align}
So the Softmax loss is a monotonically decreasing function of the features' $\emph{L}_{2}$-norm while being classified correctly.

We propose the novel and simple \emph{Feature-Norm-Loss} based on the proposition 3.2.

\textbf{p-Norm loss} To optimize the whole network to learn features with larger norm, we could simply use a scale layer to rescale all the features. But the scaling method treat all the features equally, which will fail to improve the margins between different classes.
\begin{align}
& \max \sum_{i=1}^{N}\| f_{i} \| + C \cdot \xi_{i}\\
& s.t.: \quad \forall j \neq y_{i}, \hspace{1mm} w_{y_k}f_{k}+b_{y_k} - w_{j}f_{k}-b_{j} > \xi_{i}; \hspace{3mm} \xi_{i} >= 0 \notag 
\end{align}
where $\xi_{i}$ is the slack variable, and the C is the constant factor. 
We propose the novel 3M-Softmax to improve the softmax loss based on the following two propositions. \\

\textbf{Proposition 3.1} \emph{Fixing the weight vectors and bias vectors, the Softmax loss is a monotonically decreasing function with the decreasing of the angles between the features $f_i$  and its corresponding weight vectors $w_{y_i}$ if the $x_{i}$ has been correctly classified.}

% \textbf{\emph{Proof:}} 
%Let $\mathcal{L}_{Softmax}(i, {\theta}_{w_{j}, f_{i}})$ refer the loss of the $x_i$ with the angle between $f_{i}$ and every $\{w_j\}_{K}$. Here we only offer the proof when $K=2$ and $f_{i}, w{i}, b{i}$, for $x_{i}$ of class 1. 
% \begin{align}
% \mathcal{L}_{Softmax}(k, {\theta}_{w_{1}, f_{k}})&=-log\bigg( \frac {exp(\| w_{1} \| \| f_{k} \| cos({\theta}_{w_{1}, f_{k}}) + b_{1})} {exp(\| w_{1} \| \| f_{k} \| cos({\theta}_{w_{1}, f_{k}}) + b_1) + exp(\| w_{2} \| \| f_{k} \| cos({\theta}_{w_{2}, f_{k}}) + b_2)} \bigg) 
% \end{align}

\textbf{Proposition 3.2} \emph{By fixing the weight vectors and bias, the Softmax loss is a monotonically decreasing function with the increasing of the features' norm assuming the softmax loss already could classify the samples correctly by fixing all the other variables.}

\textbf{\emph{Proof.}} Let $\mathcal{L}_{Softmax}(i, f_i)$ refer the loss of the $x_i$ with feature $f_i$, then for $\mathcal{L}_{Softmax}(k, f_k)$ for all $k = 1 \cdots N$. We have,

\begin{footnotesize}
\begin{align}
\mathcal{L}_{Softmax}(k, f_k)&=-log\bigg( \frac {exp(\| w_{y_k} \| \| f_{k} \| cos({\theta}_{w_{y_k}, f_{k}}) + b_{y_k})} {\sum_{j=1}^{K}exp(\| w_{j} \| \| f_{k} \| cos({\theta}_{w_{j}, f_{k}}) + b_k)} \bigg)  \notag \\
&= -log\bigg( \frac {1} {\sum_{j=1}^{K}exp(\| f_{k} \| (\| w_{j} \| cos({\theta}_{w_{j}, f_{k}}) + b_k - \| w_{y_k} \| cos({\theta}_{w_{y_k}, f_{k}}) - b_{y_k}))} \bigg)
\end{align}
\end{footnotesize}

Recall that the $x_{k}$ is correctly classfied, so we have $w_{y_k}f_{k}+b_{y_k} > w_{j}f_{k}+b_{j}$ for any $j \neq y_{k}$. Then $\| f_{k} \| (\| w_{j} \| cos({\theta}_{w_{j}, f_{k}}) + b_k - \| w_{y_k} \| cos({\theta}_{w_{y_k}, f_{k}}) - b_{y_k}) < 0$ always holds. So we have for any $t > 0$, 

\begin{align}
\mathcal{L}_{Softmax}(k, (1 + t)f_k) < \mathcal{L}_{Softmax}(k, f_k)
\end{align}
if we keep the $\| w_{j} \|$ and $cos({\theta}_{w_{j}, f_{k}})$ fixed. By considering all the $x_{i}$, we have ($t_k > 0$ for $k = 1 \cdots N$)
\begin{align}
\sum_{k=1}^{N} \mathcal{L}_{Softmax}(k, (1 + t_k)f_k) < \sum_{k=1}^{N} \mathcal{L}_{Softmax}(k, f_k)
\end{align}
So the Softmax loss is a monotonically decreasing function of the features' $\emph{L}_{2}$-norm while being classified correctly.

We propose the novel and simple \emph{Feature-Norm-Loss} based on the proposition 3.2.

\textbf{p-Norm loss} To optimize the whole network to learn features with larger norm, we could simply use a scale layer to rescale all the features. But the scaling method treat all the features equally, which will fail to improve the margins between different classes.
\begin{align}
& \max \sum_{i=1}^{N}\| f_{i} \| + C \cdot \xi_{i}\\
& s.t.: \quad \forall j \neq y_{i}, \hspace{1mm} w_{y_k}f_{k}+b_{y_k} - w_{j}f_{k}-b_{j} > \xi_{i}; \hspace{3mm} \xi_{i} >= 0 \notag 
\end{align}
where $\xi_{i}$ is the slack variable, and the C is the constant factor. 

==> chap/old_related_work.tex <==
\section{Related work}

We define the training dataset as $\{x_i\}_{N}$, the labels set as $\{y_i\}_{N}$ and $y_{i} = 1\dots K$ if we have N samples of K different classes. $\{f_i\}_{N}$ is the features set of $\{x_i\}_{N}$ before the softmax loss. $\{w_j\}_{K}$ is used to represent the K different class dependent weight vectors in the softmax loss. $\| v \|$ represents the $\emph{L}_{2}$$-norm$ of vector $v$.

\subsection{Softmax Loss}
The original softmax loss is defined as in equation \eqref{softmax_loss}
\begin{align}
\mathcal{L}_{softmax}=\sum_{i=1}^{N}-log\bigg( \frac {exp(w_{y_i}f_{i}+b_{y_i})} {\sum_{j=1}^{K}exp(w_{j}f_{i} + b_{j})} \bigg) \label{softmax_loss}
\end{align}
The $cos({\theta}_{w_{j}, f_{i}})$ represents the angle between the $w_{j}$ and $f_{i}$), so inner product between $w_{j}$ and $f_{i}$ can be also replaced with equation \eqref{cos}. 
\begin{align}
w_{j}f_{i} = \| w_{j} \| \| f_{i} \| cos({\theta}_{w_{j}, f_{i}}) \label{cos}
\end{align}
By combining the above 2 equations, we get 
\begin{align}
\mathcal{L}_{Softmax}=\sum_{i=1}^{N}-log\bigg( \frac {exp(\| w_{y_i} \| \| f_{i} \| cos({\theta}_{w_{y_i}, f_{i}}) + b_{y_i})} {\sum_{j=1}^{K}exp(\| w_{j} \| \| f_{i} \| cos({\theta}_{w_{j}, f_{i}}) + b_j)} \bigg) \label{softmax_loss_cos}
\end{align}
\subsection{Large Margin Softmax Loss}
The L-Softmax \ [1] is by incorporating a preset constant $m$ multiplying the angle between sample and the corresponding weight vector. 
\begin{footnotesize}
\begin{align}
\mathcal{L}_{L-Softmax}&=\sum_{i=1}^{N}-log\bigg( \frac {exp(\| w_{y_i} \| \| f_{i} \| \psi({\theta}_{w_{y_i}, f_{i}}))} {exp(\| w_{y_i} \| \| f_{i} \| \psi({\theta}_{w_{y_i}, f_{i}})) + \sum_{j=1, j \ne{y_i}}^{K}exp(\| w_{j} \| \| f_{i} \| cos({\theta}_{w_{j}, f_{i}}))} \bigg)  \label{l-softmax_loss} \\
s.t. \quad  \psi(\theta) &= (-1)^{k}cos(m\theta)-2k, \theta \in \lbrack \frac{k\pi}{m}, \frac{(k+1)\pi}{m}\rbrack  \nonumber
\end{align}
\end{footnotesize}

The L-Softmax loss has good geometric interpretaion. $m$ is used to controls the margin among classes. However, it is mentioned that when L-Softmax loss used to train datasets with too many classes, the convergence of L-Softmax will be more difficult than softmax loss. Liu W et al.\ [1] showed that L-Softmax enhanced the intra-class compactness and enlarged the inter-class separability. By replacing the inner product with cosine similarity in equation \eqref{l-softmax_loss}, Liu W et al. proposed the A-Softmax loss:
\begin{footnotesize}
\begin{align}
\mathcal{L}_{A-Softmax}&=\sum_{i=1}^{N}-log\bigg( \frac {exp(\| f_{i} \| \psi({\theta}_{w_{y_i}, f_{i}}))} {exp(\| f_{i} \| \psi({\theta}_{w_{y_i}, f_{i}})) + \sum_{j=1, j \ne{y_i}}^{K}exp(\| f_{i} \| cos({\theta}_{w_{j}, f_{i}}))} \bigg)  \label{l-softmax_loss} \\
s.t. \quad  \psi(\theta) &= (-1)^{k}cos(m\theta)-2k, \theta \in \lbrack \frac{k\pi}{m}, \frac{(k+1)\pi}{m}\rbrack  \nonumber
\end{align}
\end{footnotesize}


\subsection{Center Loss}
Wen Y et al.\ [4] proposed the center loss to simultaneously learn a center for deep features of each class and penalizes the distances between the deep features and their corresponding class centers. They showed that with the joint supervision of softmax loss and center loss, the disciminative power of the learned features can be highly enhanced. The center loss introduces a set of center features $\{c_j\}_{K}$that will be updated during the whole training procedure. Here is the defination of the center loss.
\begin{align}
\mathcal{L}_{Center-loss} = \frac{1}{2} \sum_{i=1}^{N} \| {f}_{i}-{c}_{y_i} \|_{2}^{2} \label{center_loss} \\
\mathcal{L} = \mathcal{L}_{Softmax-loss} + \frac{\lambda}{2} \mathcal{L}_{Center-loss} \label{center_softmax}
\end{align}
With the joint loss function in \eqref{center_softmax}, they achieved good accuracy on several datasets including LFW, YTF and MegaFace.

\subsection{COCO Loss / Cosine Normalization}
Chunjie L et al.\ [5] pointed that the result of dot product in the softmax loss is unbounded and increases the risk of large variance. Large variance of neuron makes the model sensitive to the change of input distribution, thus results in poor generalization. 
To solve this problem, weight normalization \ [6] reparameterizes the weight vector by dividing its norm, thus partially bounds the result of dot product. Liu Y et al.\ [4] proposed a congenerous cosine loss(\textbf{COCO}) to increase inner class similarity as well as enlarge inter-class distinction in a cooperative way. In fact, the COCO loss and the Cosine Normalization have the same form as in \eqref{COCO_loss}.

\begin{align}
\mathcal{L}_{COCO-loss} =  \sum_{i=1}^{N}-log\bigg( \frac {exp(cos({\theta}_{w_{y_i}, f_{i}}))} {\sum_{j=1}^{K}exp(cos({\theta}_{w_{j}, f_{i}}))} \bigg)\label{COCO_loss} \quad
s.t.: \quad cos({\theta}_{w_{j}, f_{i}}) = \frac{w_{j} f_{i}}{\| w_{j} \| \| f_{i} \|}
\end{align}
Experiments in [4] showed that the COCO loss can maximize the distinction across classes as well as the similarity within one class. The same ideas named cosine normalization in [5] are proven to significantly enhance the accuracy of classification and accelerate the training. 

\subsection{$\emph{L}_{2}$-Softmax Loss}
Ranjan R et al.\ [2] observed that the $\emph{L}_{2}$-norm of features learned using softmax loss is informative of the quality of the faces. Features for good quality frontal faces have a high $\emph{L}_{2}$-norm while blurry faces with extreme pose have low $\emph{L}_{2}$-norm. They argued that we should provide similar attention to both good and bad quality faces. So they proposed an $\emph{L}_{2}$-softmax loss to restrict the features to lie on a hypersphere of a fixed radius. Here is the defination of $\emph{L}_{2}$-Softmax loss

\begin{align}
\mathcal{L}_{\emph{L}_{2}-softmax}&=\sum_{i=1}^{N}-log\bigg( \frac {exp(w_{y_i} \bar{f_{i}})} {\sum_{j=1}^{K}exp(w_{j} \bar{f_{i}})} \bigg) \label{l2_softmax_loss} \\
s.t. \quad \bar{f_{i}} &= \alpha \frac{f_{i}}{\| f_{i} \|} \notag
\end{align}
They stated that the softmax loss aimed at increasing the feature norm for minimizing the overall loss. [2] also gives a bounds on the value of $\alpha $ for achieving a consistent performance. Wang F [6] proposed a similar loss function by requiring both the weight vectors and the features to lie on a hypersphere of a fixed radius. 
